Affine modules and the Drinfeld Center

Given a finite index subfactor, we show that the {\em affine morphisms at zero level} in the affine category over the planar algebra associated to the subfactor is isomorphic to the fusion algebra of the subfactor as a *-algebra. This identification paves the way to analyze the structure of affine $P$-modules with weight zero for any subfactor planar algebra $P$ (possibly having infinite depth). Further, for irreducible depth two subfactor planar algebras, we establish an additive equivalence between the category of affine $P$-modules and the center of the category of $N$-$N$-bimodules generated by $L^2(M)$; this partially verifies a conjecture of Jones and Walker.

==> texfiles/prelim.tex <==
\section{Preliminaries}\label{prelim}
\subsection{Planar algebras and subfactors}
In this section, we will recall certain basic facts about planar
algebras and subfactors, which will be used in the forthcoming
sections.  For planar algebras, we will follow the notations and
terminology used in (Section $2.1$ of) \cite{DGG} and avoid repeating
all of that in here except a few below.
\begin{enumerate}
\item We will consider the natural binary operation on $\{-,+\}$ given
  by $++ := +$, $+-:=-$, $-+:=-$ and $--:=+$.
\item We will denote the set of all possible colors of discs in tangles by $\t{Col}:= \left\{ \vlon k: \vlon \in \{+,-\},\, k \in \mbb{N}_0\right\}$ where $\N_0 := \N \cup \{ 0 \}$.
\item In a tangle, we will replace (isotopically) parallel strings by
a single strand labelled by the number of strings, and an internal disc with color $\vlon k$ will be replaced by a bold dot with the sign $\vlon$ placed at the angle corresponding to the distinguished boundary components of the disc.
For example,
$\psfrag{replace}{will be replaced by}
\psfrag{2}{$2$}
\psfrag{4}{$4$} \psfrag{e}{$\vlon$}
\vcenter{\includegraphics[scale=0.2]{figures/sfpa/dot.eps}}$
\end{enumerate}
We set some notation for a set of `generating tangles' in Figure
\ref{tangles}.
\begin{figure}[h]
\psfrag{k}{$k$}
\psfrag{2k}{$2k$}
\psfrag{e}{$\vlon$}
\psfrag{-e}{$-\vlon$}
\psfrag{M}{$ M_{\vlon k} =$}
\psfrag{m}{$(\vlon k,\vlon k)\rightarrow \vlon k$}
\psfrag{1ek}{$1_{\vlon k} =$}
\psfrag{1}{$\emptyset \rightarrow \vlon k$}
\psfrag{RI}{$RI_{\vlon k} =$}
\psfrag{ri}{$\vlon k \rightarrow \vlon (k+1)$}
\psfrag{LI}{$LI_{\vlon k}=$}
\psfrag{li}{$\vlon k \rightarrow -\vlon (k+1)$}
\psfrag{Id}{$I_{\vlon k}=$}
\psfrag{id}{$\vlon k \rightarrow \vlon k$}
\psfrag{E}{$E_{\vlon (k+1)}=$}
\psfrag{jp}{$\emptyset \rightarrow \vlon (k+2)$}
\psfrag{RE}{$RE_{\vlon (k+1)} =$}
\psfrag{re}{$\vlon(k+1) \rightarrow \vlon k$}
\psfrag{LE}{$LE_{\vlon (k+1)} =$}
\psfrag{le}{$\vlon(k+1) \rightarrow -\vlon k$}
\includegraphics[scale=0.225]{figures/sfpa/tangles.eps}\caption{Generating
  tangles.}\label{tangles}
\end{figure}
If $P$ is a planar algebra, then by a $P$-{\em labelled} tangle, we
mean a tangle whose internal discs are labelled by elements of $P$
such that an internal disc of color $\vlon k$ is labelled by an
element of $P_{\vlon k}$.  Also, ${\mcal T}_{\vlon k}$ (resp., ${\mcal
  T}_{\vlon k} (P)$) will denote the set of tangles (resp.,
$P$-labelled tangles) which has $\vlon k$ as the color of the external
disc; ${\mcal P}_{\vlon k} (P)$ will be the vector space ${\mcal
  T}_{\vlon k} (P)$ as a basis.  The action of $P$ induces a linear map $P
: {\mcal P}_{\vlon k} (P) \rightarrow P_{\vlon k}$.

We now recall the notion of the {\em $n$-th cabling} of a planar
algebra $P$ with modulus $(\delta_- , \delta_+)$, denoted by $c_n
(P)$.  For a tangle $T$, let $c_n (T)$ be the tangle obtained by (a)
replacing every string by $n$ many strings parallel to it, and (b)
putting $n$ consecutive caps on the distinguished boundary component
of every negatively signed (internal or external) disc, around the
minus sign which is then replaced by a plus sign.

\noindent {\em Vector spaces:} For all colors $\vlon k$, $c_n
(P)_{\vlon k} := \t{Range} \,(P_{c_n(I_{\vlon k})})$.


\noindent {\em Action of tangles:} For all tangles $T$, $c_n (P)_T :=
\left[ \ous{n}{\prod}{l=1} \delta_{(-)^l} \right]^{- w } P_{c_n (T)}$
where $w$ is the number of negatively signed internal disc(s) of $T$.

Note that $c_1(P)$ is isomorphic to $P$, $c_m (c_n (P)) = c_{mn} (P)$
and $c_n (P)$ has modulus $\left( \ous{n}{\prod}{l=1} \delta_{(-)^l}
  \; , \; \ous{n}{\prod}{l=1} \delta_{(-)^{l+1}} \right)$.
\vspace{1mm}

Next we move to describing the interplay between planar algebras and
subfactors. For the rest of this section, let $M_{-1} := N \subset M
=: M_0$ be a subfactor with $\delta^2 : = [M:N] < \infty$ ($\delta
>0$) and $\{M_k\}_{k \geq 1}$ be a tower of basic constructions with
$\{e_k \in \mscr{P} (M_k) \}_{k \geq 1}$ being a set of Jones
projections.  For each $k \geq 1$, set $e_{[-1,k]} := \delta^{k
  (k+1)}(e_{k+1}e_k \cdots e_1) (e_{k+2} e_{k+1}\cdots e_2)\cdots
(e_{2k+1} e_{2k}$ $\cdots e_{k+1}) \in N^\prime \cap M_{2k+1}$, $
e_{[0, k]} :=\delta^{k (k-1)} (e_{k+1}e_k \cdots e_2) (e_{k+2}
e_{k+1}\cdots e_2)\cdots (e_{2k} e_{2k-1} \cdots e_{k+1}) \in M^\prime
\cap M_{2k}$ and $v_k := \delta^k e_k e_{k-1} \cdots e_1 \in N^\prime
\cap M_k$.  Then, the tower of $II_1$ factors $N \subset M_k\subset
M_{2k+1}$ (resp., $M \subset M_k \subset M_{2k}$) is an instance of
basic construction with ${e_{[-1,k]}}$ (resp., ${e_{[0,k]}}$) as Jones
projection, that is, there exists an isomorphism $ {\varphi_{-1, k}} :
M_{2k+1} {\lra} \mcal{L}_N(L^2(M_k))$ (resp., ${\varphi_{0, k}} :
M_{2k} {\lra} \mcal{L}_M(L^2(M_k))$) given by
\begin{eqnarray*}
  \varphi_{-1, k}(x_{2k+1}) \hat{x}_{k} & = & 
  \delta^{2(k+1)} E_{M_k}(x_{2k+1}x_{k}e_{[-1,k]})^{\widehat{}}  \\
  \text{(resp., } \varphi_{0,k} (x_{2k}) \hat{x}_{k} &= &
  \delta^{2k} E_{M_k}(x_{2k}x_{k}e_{[0,k]})^{\widehat{}} \text{ )}
\end{eqnarray*}
for all $x_i \in M_i$, $i = k,\, 2k,\, 2k+1$, which is identity
restricted to $M_k$ and sends $e_{[-1,k]}$ (resp., $e_{[0,k]}$) to the
projection with range $L^2(N)$ (resp., $L^2(M)$).  Also, $\varphi_{-1,
  k} (M_i'\cap M_{2k+1}) =\,_{M_i}\mcal{L}_N(L^2(M_k))$ (resp.,
$\varphi_{0, k}(M_i'\cap M_{2k}) = \, _{M_i}\mcal{L}_M(L^2(M_k))$) and
$\vphi_{0,k} = \left. \vphi_{-1,k} \right|_{M_{2k}}$ for all $k \geq 0
$, $-1 \leq i \leq k$.

We now state the `extended Jones' theorem' which provides an important
link between finite index subfactors and planar algebras. This was
first established for extremal finite index subfactors in
\cite{Jon}. Later, it was extended to arbitrary finite index
subfactors in \cite{Bur, JP, DGG}. As mentioned above, we will follow
the set up of \cite{DGG}.
\begin{thm}\label{jones-theorem}
  $P$ defined by $P_{\vlon k} = N' \cap M_{k-1} $ or $M' \cap M_{k}$
  according as $\vlon = +$ or $-$, has a unique unimodular bimodule
  planar algebra structure with the $\ast$-structure given by the
  usual $\ast$ of the relative commutants such that for each $k \in
  \N_0$,
\begin{enumerate}
\item the action of multiplication tangles is given by the usual
multiplication in the relative commutants,
\item the action of the left inclusion tangle $LI_{-k}$ is given by
  the usual inclusion $M' \cap M_k \subset N'\cap M_k$,
\item the action of the right inclusion tangle $RI_{+k}$ is given by
  the usual inclusion $ M_{k-1} \subset M_{k}$,
\item $P_{E_{+(k+1)}} = \delta e_{k+1}$,
\item $P_{LE_{+(k+1)}} = \delta^{-1} \us{i}{\sum} b_i^* x b_i $ for
  all $ x \in P_{+(k+1)}$,
\end{enumerate}
where $\{ b_i\}_i$ is a left Pimsner-Popa basis for the subfactor $N
\subset M$.  ($P$ will be referred as the planar algebra associated to
the tower $\{M_k\}_{k \geq -1}$ with Jones projections $\{e_k\}_{k
  \geq 1}$.)
\end{thm}
\begin{rem}\label{jones-theorem-rem}
  Apart from the action of the tangles given in conditions (1) - (5),
  it is also worth mentioning the actions of a few other useful
  tangles, namely,

(a) $P_{RE_{+k}} = \delta \left. E^{M_{k-1}}_{M_{k-2}}
\right|_{P_{+k}}$,

(b) $P_{TR^r_{+k}} = \delta^k \left. tr_{M_{k-1}} \right|_{P_{+k}}$,

(c) $\delta^{-k} P_{TR^l_{+{2l}}}$ (resp., $\delta^{-k}
P_{TR^l_{+(2l-1)}}$) is given by the trace on $P_{+2l} = N' \cap
M_{2l-1}$ (resp., $P_{+(2l-1)} = N' \cap M_{2l-2}$) induced by the
canonical trace on ${_N} {\mcal L} ( L^2 (M_{l-1}) )$ via the map
$\vphi_{-1,l-1}$ (resp., $\vphi_{0,l-1}$).
\end{rem}
\begin{cor}\label{dualpa}
  (a) $P_{E'_{-k}} (y) = \delta \us{i}{\sum} b^*_i e_1 y e_1 b_i$ for
  all $y \in P_{-k} = M' \cap M_k$, where $E'_{-k} = LI_{+(k-1)} \circ
  LE_{-k}$ and $\{ b_i \}_i$ is a left Pimsner-Popa basis for $N
  \subset M$,

  (b) the $n$-th dual of $P$, $\lambda_n (P) =$ the planar algebra
  associated to the tower $\{ M_{k+n} \}_{k \geq -1}$ with Jones
  projections $\{ e_{k+n} \}_{k \geq 1}$.
\end{cor}
If $e_{[l,k+l]}$ denotes the projection obtained by replacing each
$e_\bullet$ in the defining equation of $e_{[0,k]}$ (as above), by
$e_{l+\bullet}$, then $M_l \subset M_{k+l} \subset M_{2k+l}$ is an
instance of basic construction with $e_{[l,k+l]}$ as Jones projection.
\begin{rem}\label{cabling}
  An easy consequence of Corollary \ref{dualpa} (b) and Theorem
  \ref{jones-theorem} is $c_n(P) =$ the planar algebra associated to
  the tower $\{ M_{n(k+1)-1} \}_{k \geq -1}$ with Jones projections
  $\{e_{[n(k-1)-1,nk-1]} \}_{k \geq 1}$.
\end{rem}
\begin{prop}\label{rotcont} 
  If $J_k$ denotes the canonical conjugate-linear unitary operator on
  $L^2 (M_k)$ and $R^m_{\vlon n}$ denotes the tangle
  \psfrag{e}{$\vlon$} \psfrag{m}{$m$} \psfrag{2n-m}{$2n-m$}
  \psfrag{-e}{$(-)^m \vlon$}
\includegraphics[scale=0.2]{figures/sfpa/rot.eps}
, then for all $k \geq 0$, we have:

(a) $\vphi_{-1,k} \left( P_{R^{2k+2}_{+(2k+2)}} (x) \right) = J_k
\vphi_{-1,k} (x^*) J_k \;$ and $\; \t{Range} \,
\vphi_{-1,k} \left( P_{R^{2k+2}_{+(2k+2)}} (p) \right) \os{N \text{-}
  N}{\cong} \oline{\t{Range} \,\vphi_{-1,k} (p)}$ for all $x \in P_{+(2k+2)}$, $p \in {\mathscr P}
(P_{+(2k+2)})$,

(b) $\vphi_{-1,k} \left( P_{R^{2k+1}_{+(2k+1)}} (x) \right) = J_k
\vphi_{0,k} (x^*) J_k \;$ and $\; \t{Range} \,
\vphi_{-1,k} \left( P_{R^{2k+1}_{+(2k+1)}} (p) \right)$$\os{M \text{-}
  N}{\cong}$$\oline{\t{Range} \,\vphi_{-1,k} (p)}$ for all $x \in P_{+(2k+1)}$, $p \in {\mathscr P}
(P_{+(2k+1)})$,

(c) $\vphi_{0,k} \left( P_{R^{2k+1}_{-(2k+1)}} (x) \right) = J_k
\vphi_{-1,k} (x^*) J_k \;$ and $\; \t{Range} \,
\vphi_{0,k} \left( P_{R^{2k+1}_{-(2k+1)}} (p) \right) \os{N \text{-}
  M}{\cong} \oline{\t{Range} \,\vphi_{-1,k} (p)}$ for all $x \in P_{-(2k+1)}$, $p \in {\mathscr P}
(P_{-(2k+1)})$,

(d) $\vphi_{0,k} \left( P_{R^{2k}_{-2k}} (x) \right) = J_k \vphi_{0,k}
(x^*) J_k \;$ and $\; \t{Range} \,\vphi_{0,k} \left(
  P_{R^{2k}_{-2k)}} (p) \right) \os{M \text{-} M}{\cong} \oline{\t{Range} \,
  \vphi_{0,k} (p)}$ for all $x \in P_{-2k}$, $p \in {\mathscr P} (P_{-2k})$.
\end{prop}
\begin{pf}
  The isomorphism in the second part in each of (a), (b), (c) and (d),
  follows from the first part using \cite[Proposition $3.11$]{Bis97}.
  For the first parts, it is enough to establish only for (a) because
  all others can be deduced using conditions (2) and (3) in Theorem
  \ref{jones-theorem}, and the relation $\vphi_{0,k} =
  \left. \vphi_{-1,k} \right|_{M_{2k}}$.

  First, we will prove part (a) for $k=0$.  Note that if $\{b_i\}_i$
  is a left Pimsner-Popa basis for $N \subset M$, then
 \[
P_{R^2_{+2}} (x) = P_{R^1_{-2}} \left( P_{R^1_{+2}} (x) \right) =
P_{R^1_{-2}} \left( \delta \us{i}{\sum} b^*_i x e_2 e_1 b_i \right) =
\delta^4 \us{i}{\sum} E_{M_1} \left( e_2 e_1 b^*_i x e_2 e_1 b_i \right)
\]
where we use the conditions of Theorem \ref{jones-theorem} in a
decomposition of the rotation tangle into the generating ones $R^1_{+2}
= LE_{+3} \circ M_{+3} ( RI_{+2} , M_{+3} (E_{+2} , RI_{+2} \circ
E_{+1}) )$ (resp., $RE_{+3} \circ M_{+3} (M_{+3} (E_{+2} , RI_{+2}
\circ E_{+1}) , LI_{-2})$) for establishing the second (resp., third)
equality. For $y \in M$, note that
\begin{align*}
\vphi_{-1,0} \left( P_{R^2_{+2}} (x) \right) \hat{y} & =
\delta^6 \sum_i E_M ( e_2 e_1 b_i^* x e_2 e_1 b_i y e_1 ) \hat{}
= \delta^6 E_M ( e_2 e_1 y x
e_2 e_1 ) \hat{} = \delta^2 E_M (e_1 y x)\hat{}\\
& = J_0 \vphi_{-1, 0}
(x^*) J_0 \hat{y}.
\end{align*}
Now, let $k > 0$. Using the above and
Remark \ref{cabling}, we obtain
\[
\vphi_{-1,k} \left( P_{R^{2k+2}_{+(2k+2)}} (x) \right) = \vphi_{-1,k} \left( {c_{k+1}(P)}_{R^2_{+2}} (x) \right) = J_k \vphi_{-1 , k} (x^*) J_k.
\]
\end{pf}
\vspace{2mm}

We will make repeated use of the following standard facts, whose proof
can be found in \cite{Bis97}.
\begin{lem} \cite{Bis97}\label{e-even-odd}
For each $k \geq 0$, and $ X \in \{N, M\}$, we have:
\begin{enumerate}
\item $\t{Range} \,\varphi_{-1, k} (p) \os{X-N}{\cong} \t{Range} \,\varphi_{-1, k+1}
  (pe_{2k+3})$ for all $p \in \mscr{P} (X' \cap M_{2k +1})$,
\item $\t{Range} \,\varphi_{0, k} (p) \stackrel{X-M}{\cong} \t{Range} \,\varphi_{0,
    k+1} (pe_{2k+2})$ for all $p \in \mscr{P} (X' \cap M_{2k})$.
\end{enumerate}
\end{lem}
\noindent From this, one can easily deduce the following.
\begin{cor}\label{p-q-equivalence}
For $k > l \geq 0$ and $X \in \{N, M\}$, the following holds:
\begin{enumerate}
\item For all $p \in \mscr{P} (X' \cap M_{2k +1})$ and $q \in \mscr{P}
  (X' \cap M_{2l + 1})$ satisfying $\t{Range} \,\varphi_{-1, k} (p)
  \stackrel{X-N}{\cong} \t{Range} \,\varphi_{-1, l} (q)$, $p$ is
  MvN-equivalent to $q e_{2l+3}\cdots e_{2k+1}$ in $X' \cap M_{2k +
    1}$.
\item For all $p \in \mscr{P} (X' \cap M_{2k})$ and $q \in \mscr{P}
  (X' \cap M_{2l})$ satisfying $\t{Range} \,\varphi_{0, k} (p)
  \stackrel{X-M}{\cong} \t{Range} \,\varphi_{0, l} (q)$, $p$ is MvN-equivalent
  to $q e_{2l+2}\cdots e_{2k}$ in $X' \cap M_{2k}$.
\end{enumerate}
\end{cor}
\subsection{Affine Category over a  Planar Algebra}\label{affrep}
In this subsection, for the sake of self containment, we recall (from
\cite{Gho}) in some detail what we mean by the \textit{affine category
  over a planar algebra} and the corresponding {\em affine morphisms}
(with slight modifications).
\begin{defn}
  For each $ \varepsilon , \eta \in \{ +, - \}$ and $k, l \geq 0$, an
  $(\varepsilon k , \eta l)$-affine tangular picture consists of the
  following:
\begin{itemize}
\item finitely many (possibly none) non-intersecting subsets $D_{1},
  \cdots , D_{b}$ (referred as disc(s)) of the interior of the
  rectangular annular region $RA:= [-2, 2]\times [-2, 2] \setminus
  (-1, 1)\times (-1, 1)$, each of which is homeomorphic to the unit
  disc and has even number of marked points on its boundary, numbered
  clockwise,
\item non-interescting paths (called strings) in $RA \setminus \left[
    \ous{b}{\sqcup}{i=1} \mathrm{Int} (D_i) \right]$, which are either
  loops or meet the boundaries of the discs or $RA$ exactly at two
  distinct points in $\{ (\frac{i}{2k}, 1): 0 \leq i \leq 2k-1\}
  \sqcup \{ (\frac{j}{2l}, 2) : 0 \leq j \leq 2l-1\} \sqcup
  \{\text{marked points on the discs} \}$ in such a way that every
  point in this set must be an endpoint of a string,
\item a checker-board shading on the connected components of $Int(RA)
  \setminus \left[ \left( \ous{b}{\sqcup}{i=1} D_i\right)\, \cup
    \{\mathrm{strings}\, \} \right]$ such that the component near the
  point $(0,-1)$ (resp., $(0,-2)$) is unshaded or shaded according as
  $\vlon$ (resp., $\eta$) is $+$ or $-$.

\end{itemize}
\end{defn}
\begin{defn}\label{aff-isotopy}
  An affine isotopy of an affine tangular picture is a map $\varphi :
  [0, 1] \times RA \ra RA$ such that
\begin{enumerate}\vspace*{-2mm}
\item $\varphi(t, \cdot)$ is a homeomorphism of $RA$, for all $t \in
  [0, 1]$;
\item $\varphi(0, \cdot) = id_{RA}$; and
\item $\left. \varphi(t, \cdot) \right|_{\partial (RA)} = id_{\partial
    (RA)}$ for all $t \in [0, 1]$.
\end{enumerate}
\end{defn}
Two affine tangular pictures are said to be {\em affine isotopic} if
one can be obtained from the other using an affine isotopy preserving
checker-board shading and the distinguished boundary components of the
discs.
\begin{defn}
  An $(\varepsilon k , \eta l )$-affine tangle is the affine isotopy
  class of an $(\varepsilon k , \eta l )$-affine tangular picture.
\end{defn}
Time and again, for the sake of convenience, we will abuse terminology
by referring an affine tangular picture as an affine tangle
(corresponding to its affine isotopy class) and the figures might not
be sketched to the scale but are clear enough to avoid any ambiguity.
In Figure \ref{aff-tangles}, we draw a specific affine tangle called
$\Psi_{\varepsilon k, \vlon^m l}^m$, where a number beside a string
has the same meaning as in tangles.  This affine tangle will play an
important role in the following discussions.
\begin{figure}[h]
\psfrag{AR}{$AR_{\vlon k}$}
\psfrag{y}{$\eta$}
\psfrag{2k-1}{$2k-1$}
\psfrag{2k}{$2k$}
\psfrag{2l}{$2l$}
\psfrag{m}{$m$}
\psfrag{e}{$\varepsilon$}
\psfrag{-e}{$-\varepsilon$}
\psfrag{psi}{$\Psi^m_{\varepsilon k, \eta l}$}
\psfrag{1ek}{$A1_{\varepsilon k}$}
\includegraphics[scale=0.30]{figures/affcat/afftang.eps}
\caption{Some useful affine tangles. ($\varepsilon , \eta \in \{+, -
  \}, k, l \in \N_0, m \in (2\N_0 + \delta_{\vlon \neq
    \eta})$) \label{aff-tangles}}
\end{figure}

\noindent {\bf Notations:} For each $ \varepsilon , \eta \in \{ +, -
\}$ and $k, l \geq 0$, let $\mathcal{AT}_{\varepsilon k, \eta l}$
denote the set of all $(\varepsilon k, \eta l)$-affine tangles, and
let $\mcal{A}_{\varepsilon k, \eta l}$ denote the complex vector space
with $\mcal{AT}_{\varepsilon k, \eta l}$ as a basis.  The composition
of affine tangles $T \in \mathcal{AT}_{\varepsilon k, \eta l}$ and $S
\in \mathcal{AT}_{\xi m, \varepsilon k}$ is given by $T \circ S :=
\frac{1}{2}(2T \cup S) \in \mcal{AT}_{\xi m , \eta l}$; this
composition is linearly extended to the level of the vector spaces
$\mcal{A}_{\vlon k, \eta l}$'s.

\begin{rem} \label{Psi-remark}
For each $A \in \mathcal{AT}_{\varepsilon k, \eta l}$, there is an $m \in (2\mbb{N}_0 + \delta_{\vlon \neq \eta})$ and a  $T \in \mcal{T}_{\eta(k + l +m)}$ such that $A = \Psi_{\varepsilon k, \eta l}^m (T)$ where $\Psi_{\varepsilon k, \eta l}^m (T)$ is the isotopy class of the affine tangular picture obtained by inserting $T$ in the disc of $\Psi_{\varepsilon k, \eta l}^m$.
\end{rem}
In the above remark, the $m$ can be chosen as large as one wants and the insertion method extends linearly to a linear map $\Psi_{\vlon k, \eta l}^m : \mcal{P}_{\eta (k + l + m)} \ra \mcal{A}_{\varepsilon k, \eta l}$, and for each $A \in \mathcal{A}_{\varepsilon k, \eta l}$, there is an $m \in \mbb{N}_0 $ and an $X \in \mcal{P}_{\eta(k + l +m)}$ such that $A = \Psi_{\varepsilon k, \eta l}^m (X)$.  Let $P$ be a planar algebra.
An $( \varepsilon k, \eta l)$-affine tangle is said to be $P$-{\em labelled} if each disc is labelled by an element of $P_{\xi m}$ where $\xi m$ is the color of the disc.
Let $\mathcal{AT}_{\varepsilon k, \eta l}(P)$ denote the collection of all $P$-{\em labelled} $(\varepsilon k, \eta l)$-affine tangles, and let $\mathcal{A}_{\varepsilon k, \eta l}(P)$ be the vector space with $\mathcal{AT}_{\varepsilon k, \eta l}(P)$ as a basis.
Composition of $P$-{\em labelled} affine tangles also makes sense as above and extends to their complex span.
Note that $\Psi_{\varepsilon k, \eta l}^m$ also induces a linear map from $\mathcal{P}_{\eta (k+l+m)}(P)$ into $\mathcal{A}_{\varepsilon k, \eta l}(P)$.
Moreover, from \ref{Psi-remark}, we may conclude that, for each $A \in \mathcal{A}_{\varepsilon k, \eta l}(P)$, there is an $m \in (2\mbb{N}_0 + \delta_{\vlon \neq \eta})$ and an $X \in \mcal{P}_{\eta(k + l +m)}(P)$ such that $A = \Psi_{\varepsilon k, \eta l}^m (X)$.

\vspace{2mm}
Now, consider the set $\mathcal{W}_{\varepsilon k,\eta l} := \us{m \in
  \N_0}{\cup} \left\{ \Psi _{\varepsilon k, \eta l }^{m}(X) : X \in
  \mathcal{P}_{\eta (k+l+m)}(P) \text{ s.t. } P_X = 0 \right\}$. It is
straight forward - see \cite{Gho} - to observe that
$\mathcal{W}_{\varepsilon k,\eta l}$ is a vector subspace of
$\mathcal{A}_{\varepsilon k, \eta l}(P)$.

Define the category $AP$ by:
\begin{itemize}
\item $\text{ob}(AP) := \{\varepsilon k : \varepsilon \in \{+,-\}, k\in
  \mathbb{N}_{0}\}$,
\item $\text{Mor}_{AP}(\varepsilon k, \eta l) :=
  \frac{\mathcal{A}_{\varepsilon k,\eta l}
    (P)}{\mathcal{W}_{\varepsilon k, \eta l}}$ (also denoted by
  $AP_{\varepsilon k,\eta l}$),
\item composition of morphisms is induced by the composition of
  $P$-{\em labelled} affine tangles (see \cite{Gho}),
\item the identity morphism of $\varepsilon k$ is given by the class
  $[A1_{\varepsilon k}]$ - Figure \ref{aff-tangles}.
\end{itemize}
$AP$ is a $\mbb C$-linear category and is called the \textit{affine category over $P$} and the morphisms in this category are called {\em affine morphisms}.

For $\vlon k, \eta l \in \t{Col}$ and $m \in (2\N_0 + \delta_{\vlon \neq \eta})$, consider the composition map
\[
\psi_{\vlon k , \eta l}^{m} \; : \; P_{\eta (k+l+m)} \stackrel{ I_{\eta (k+l+m)}}{\lra} \mcal{P}_{\eta (k+l+m)}(P) \stackrel{ \Psi^m_{\vlon k, \eta l}}{\lra} \mcal{A}_{\vlon k, \eta l}(P) \stackrel{q_{\vlon k, \eta l}}{\ra} AP_{\vlon k, \eta l}
\]
where the map $I_{\eta (k+l+m)} : P_{\eta (k+l+m)} \ra \mcal{P}_{\eta (k+l+m)}(P)$ is obtained by labelling the internal disc of the identity tangle $I_{\eta (k+l+m)}$ (defined in Figure \ref{tangles}) by a vector in $P_{\eta (k+l+m)}$, and $q_{\vlon k , \eta l}: \mcal{A}_{\vlon k, \eta l}(P) \ra AP_{\vlon k, \eta l}$ is the quotient map. Note that $\psi^m_{\vlon k, \eta l}$ is indeed linear, although $I_{\eta (k+l+m)}$ is not.
\begin{rem}\label{psi-remark}
For each $a \in AP_{\vlon k, \eta l}$, there exists $m \in (2\mbb{N}_0 + \delta_{\vlon \neq \eta})$ and  $x \in P_{\eta(k + l +m)}$ such that $a = \psi_{\vlon k, \eta l}^m (x)$.
\end{rem}

Note that if $P$ is a $\ast $-planar algebra, then each $\mathcal{P}_{\varepsilon k }(P)$ becomes a $\ast $-algebra where $\ast $ of a {labelled} tangle is given by $\ast $ of the unlabelled tangle whose internal discs are labelled with $\ast$ of the labels.
Further, one can define $\ast$ of an affine tangular picture by reflecting it inside out such that the reflection of the distinguished boundary segment of any disc becomes the same for the disc in the reflected picture; this also extends to the $P$-{\em labelled} affine tangles as in the case of $P$-{\em labelled} tangles.
Clearly, $\ast$ is an involution on the space of $P$-affine tangles, which can be extended to a conjugate linear isomorphism $\ast : \mcal{A}_{\varepsilon k, \eta l} (P) \rightarrow \mcal{A}_{\eta l ,  \varepsilon k} (P)$ for all colours $\varepsilon k$, $\eta l$.
Moreover, it is readily seen that $\ast \left( \mathcal{W}_{\varepsilon k, \eta l}\right) =\mathcal{W}_{\eta l,\varepsilon k}$; so the category $AP$ inherits a $\ast$-category structure.

A $\C$-linear functor $V$ from $AP$ to $\mcal{V}ec$ (the category of complex vector spaces), is said to be an {\em affine $P$-module}, that is, there exists vector spaces $V_{\vlon k}$'s and linear maps sending an affine morphism $a \in AP_{\vlon k , \eta l}$ to its action $ V_a \in \text{Mor}_{\mcal{V}ec} (V_{\vlon k} , V_{\eta l}) $ for $\vlon k , \eta l \in \text{Col}$ such that compositions and identities are preserved.
For a $*$-planar algebra $P$, we will be interested in {\em $*$-affine $P$-modules} preserving the $*$-structure of $AP$, that is, they will be given by $\C$-linear functors $V$ from $AP$ to the category of inner product spaces such that $\langle \xi , a \eta \rangle = \langle a^* \xi , \eta \rangle$ for all affine morphisms $a$, and $\xi$ and $\eta$ in appropriate $V_{\vlon k}$'s; $V$ will be called {\em Hilbert affine $P$-module} if $V_{\vlon k}$'s are Hilbert spaces.
Moreover, affine modules are called {\em bounded} (resp., {\em locally finite}) if the actions of the affine morphisms are bounded operators with respect to the norm coming from the inner product (resp., $V_{\vlon k}$'s are finite dimensional).
By closed graph theorem, a Hilbert affine $P$-module is automatically bounded; conversely, every bounded $*$-affine $P$-module could be completed to a Hilbert affine module.

Below, we give a list of some standard facts on Hilbert affine $P$-modules for a $*$-planar algebra $P$ with modulus.
If $V$ is a Hilbert affine $P$-module and $S_{\vlon k}\subset V_{\vlon k}$ for $\vlon k\in\mbox{Col}$, then one can consider the `submodule of $V$ generated by $S=\us{\vlon k\in\mbox{Col}}{\coprod}S_{\vlon k}$' given by $\left\{ \left[S\right]_{\eta l}:=\ol{\mbox{span}\left\{ \us{\varepsilon k\in\mbox{Col}}{\cup}AP_{\vlon k,\eta l}\left(S_{\varepsilon k}\right)\right\} }^{\parallel\cdot\parallel}\right\} _{\eta l}$ which
is also the smallest submodule of $V$ containing $S$.
\begin{rem}\label{irrmod}
Let $V$ be a Hilbert affine $P$-module and $W$ be an $AP_{\vlon k,\vlon k}$-submodule
of $V_{\vlon k}$ for some $\vlon k\in\mbox{Col}$. Then,
\begin{enumerate}
\item $V$ is irreducible if and only if $V_{\vlon k}$ is irreducible $AP_{\vlon k,\vlon k}$-module
for all $\vlon k\in\mbox{Col}$ if and only if $\left[v\right]=V$
for all $0\neq v\in V$.
\item $W$ is irreducible $\Leftrightarrow$ $\left[W\right]$ is an irreducible
submodule of $V$.\end{enumerate}
\end{rem}
\begin{rem}\label{affmodmor}
If $V$ and $W$ are Hilbert affine $P$-modules such that there exists
an $\vlon k\in\mbox{Col}$ $AP_{\vlon k,\vlon k}$-linear isometry
$\theta:V_{\vlon k}\ra W_{\vlon k}$ and $V=\left[V_{\vlon k}\right]$,
then $\theta$ extends uniquely to an isometry $\tilde{\theta}:V\ra W$.
\end{rem}
For $\vlon=\pm,$ we will also consider \emph{Hilbert $\vlon$-affine
$P$-module} $V$ consisting of the Hilbert spaces $V_{\pm0},V_{1},V_{2},\ldots$
and with an action of affine morphism from $AP_{\vlon k,\vlon l}$
for $k,l\in\N$ and $AP_{\eta0,\nu0}$ for $\eta,\nu\in\left\{ \pm\right\} $
such that the action preserves $*$.
\begin{rem}\label{eaff}
The restriction map from the set of isomorphism classes of Hilbert
affine $P$-modules to that of the Hilbert $\vlon$-affine $P$-modules,
is a bijection.
\end{rem}
To see this, consider an irreducible Hilbert $+$-affine $P$-module $V$.
Define $\t{Ind} \, V_{\vlon k}:=V_{k}$ and $\t{Ind} \, V_{\vlon0}:=V_{\vlon0}$
(as Hilbert spaces) and the action of affine morphisms by  $AP_{\vlon k,\eta l}\times \t{Ind} \, V_{\vlon k} \ni (a,v) \longmapsto \left(r_{\eta l}^{-1}\circ a\circ r_{\vlon k}\right)\cdot v\in \t{Ind} \, V_{\eta l}$
where $r_{\vlon k}=\left\{ \begin{array}{ll}
A1{}_{\vlon k}, & \mbox{ if }k=0\mbox{ or }\vlon=+,\\
AR_{\vlon k}, & \mbox{ otherwise.}\end{array}\right.$

For every affine $P$-module $V$, $\mbox{dim}\left(V_{+k}\right)=\mbox{dim}\left(V_{-k}\right)$ for all $k\geq1$ and it increases as $k$ increases.
\emph{Weight of $V$} is defined as the smallest non-negative integer $k$ such that $V_{+k}$ or $V_{-k}$ is nonzero.
